Connecting Web Event Forecasting with Anomaly Detection: A Case Study on Enterprise Web Applications Using Self-Supervised Neural Networks

Recently web applications have been widely used in enterprises to assist employees in providing effective and efficient business processes. Forecasting upcoming web events in enterprise web applications can be beneficial in many ways, such as efficient caching and recommendation. In this paper, we present a web event forecasting approach, DeepEvent, in enterprise web applications for better anomaly detection. DeepEvent includes three key features: web-specific neural networks to take into account the characteristics of sequential web events, self-supervised learning techniques to overcome the scarcity of labeled data, and sequence embedding techniques to integrate contextual events and capture dependencies among web events. We evaluate DeepEvent on web events collected from six real-world enterprise web applications. Our experimental results demonstrate that DeepEvent is effective in forecasting sequential web events and detecting web based anomalies. DeepEvent provides a context-based system for researchers and practitioners to better forecast web events with situational awareness.

==> 1_intro.tex <==
Web applications provide extended connectivity to an organization's assets and increase the attack surface of its web-facing infrastructure. They have become favorite targets of cyber-attacks due to easy access and constantly increasing vulnerabilities. Anomaly detection is a critical component to protect web applications against cyber threats. Supervised learning~\cite{kruegel2003anomaly,pham2016anomaly,dong2017adaptively,yu2018deephttp} and unsupervised learning~\cite{zolotukhin2014anomaly,Juvonen12015anomaly} have been proposed to analyze web requests for anomaly detection.
Supervised learning based solutions build detection systems by discovering abnormal behavioral patterns with the use of labeled training data. 
Unfortunately, high quality annotated data is not easy to obtain, given the velocity, volume, and real-time nature of web requests. 
Usually, labeled data are very imbalanced as it is hard to collect a large number of labeled anomalies as opposed to normal web requests. 
Insufficient and imbalanced training data hinder the performance of machine learning models~\cite{japkowicz2002}. 
Limited labeled data from previous attacks undercut the ability to use supervised models, and constantly evolving attacks make such supervised models irrelevant. 
On the other hand, unsupervised learning based solutions can analyze data without labels, but they are often prone to low accuracy and high false positives, which means that such solutions may flag a benign web request as anomalous or, conversely, an attack as a normal request. 

In addition, previous studies focus on detecting anomalies based on the content of individual web request. Kruegel~\etal, Tapiador~\etal, and Robertson~\etal investigated the textual information conveyed in web requests and analyzed features from URI paths and parameters~\cite{kruegel2003anomaly,et2004anomaly,robertson2006using}. Recently, Liang~\etal, Yu~\etal, and Liu~\etal train neural networks based on every character in a web request~\cite{liang2017anomaly,yu2018deephttp,liu2019locate}. While doing so is useful to understand if a single web request is normal or not, they do not capture the relationship among the web requests.
% Although doing so is useful to understand a single web request, these methods do not capture the relationship among the web requests.
However, the methods analyzing a single web request cannot capture the relationship among the sequential web requests, which provides more useful information for anomaly detection such as user behaviors, web application flow characteristics. 
For example, authentication mechanisms (\eg, OpenID Connect, OAuth 2.0, API-token) allow us to identify the user who generates web requests. %Virtual private network (VPN) traces users' interactions with web applications as well. 
Hence, one can identify the anomalies deviated from users' normal patterns by tracking and analyzing the sequence of web requests based on users' footprint. In addition, each web application has its flow characteristics, \eg, the sequence of requests produced by specific actions. Web-based exploits, however, may have very different sequences of requests corresponding to different attack steps. 

Therefore, two critical challenges exist in characterizing the sequence of web requests for anomaly detection. First, less structured web requests need to be represented in a low-dimensional vector space such that their relationship can be encoded in the latent space. The format and semantics of web requests vary significantly from application to application. We need to develop techniques to automate the process of characterizing web requests and representing them in the desired vector space.

Second, the relationship between web requests is complicated. For example, browsing a web page can produce a sequence of web requests, and the length of the sequence varies a lot for different web pages. A web request is made for the HTML of the web page itself, and subsequent requests are made for each image, plug-in, audio clip, and other content referenced in the HTML. The web requests for each piece
of content increase the length of the sequence. To  illustrate this, consider a real-world example in Figure~\ref{fig:wordpress} where we performed two simple actions on a WordPress website: login
and browse the homepage. Login itself produces $4$ requests ($e1$ to $e4$), and a URI forwarding ($e5$) as well as subsequent $10$ requests ($e6$ to $e15$) are automatically generated afterward. One
web request ($e16$) is made for browsing the homepage itself, and this request is followed by another $17$ requests ($e17$ to $e33$) for each content referenced on the homepage. Give a sequence of those $33$ requests, it is not trivial to understand how $e33$ is produced together with $e1$. Considering all these temporal actions and web content dependent factors, it is desirable to have a model that is able to understand a sequence of web requests with respect to actions.


\begin{figure}[!tb]
\centering
\includegraphics[width=0.95\linewidth]{figures/wordpress.png}
\caption{HTTP Requests collected from a WordPress website.}
% \label{fig:wordpress}
\end{figure}


To address the above challenges, we design \bp, a novel context-based web request anomaly detection system. We make the following contributions in this paper:
\begin{itemize}
    \item \textit{Self-supervised learning to overcome the need for labeled data.} We formulate anomaly detection as a self-supervised learning problem~\cite{raina2007self,jing2019self} without requiring any prior knowledge of anomalous web requests' features and their sequential relationships. Self-supervised learning uses naturally existing evidence as labeled data for training, thus overcomes the need for labeled data in supervised learning. In addition, we leverage a pre-training process that learns the representations of web requests to further compensate for the lack of labeled data.
    
    \item \textit{Context-based web requests analysis.} \bp characterizes not only the individual web requests, but also the relationships among the web requests that co-occur within a context, \ie, a sequence of requests that are commonly produced together for a specific user and web applications' flow characteristics. To model the context of a web request, we leverage techniques that have been proposed in the area of Natural Language Processing (NLP) and deep neural networks. Word embedding \cite{mikolov2013distributed} provides powerful tools for modeling relationships between words. Such approaches represent words with low-dimensional vectors based on the neighboring words that appear in the same sentence (\ie, the context). These vectors can capture the context of a word and its relationship with other words in a sentence. Similarly, we calculate the embedding of a web request by considering the entire session of web requests generated by a user as a sentence, and each request as a word. Based on the context, \bp predicts the web requests that are likely to appear with associated probabilities. %An abnormal request is flagged if this request is not within the top probabilities to appear based on the model's prediction. %Context-based anomaly detection is resilient to attacks. Because adversaries have to understand the victim web application's characteristics as well as its users' behaviors to evade the detection system. 
   % We take into account the characteristics of web requests, e.g., task-critical requests may locate far from each other %(\eg, requests $e1$ and $e16$ shown in Figure~\ref{fig:wordpress}). To construct direct links between task-critical requests, we leverage neural network models to learn from the long-distance context. 
%If the target app does not have any related web applications, \ie, exogenous apps, or the web requests from the exogenous apps are not available, \bp detects anomalies using contextual events from target app, \ie, $\{e_1^{t}, e_2^{t}, \ldots, e_{n_t}^{t}\}$. 
% In the cases where there is no exogenous apps or the contextual events are not available, the model works as shown in Figure~\ref{fig:single_model}. 
    \item \textit{Quantitative measures of the anomaly.}
    Different from traditional anomaly detection methods, \bp goes beyond binary prediction. Upon encoding the relationship between web requests within the vector space, we can quantitatively predict the web requests appearing in similar contexts in the latent space. Therefore, \bp predicts if a web request belongs to normal behavior and also measures the deviation of the abnormal request with respect to expected normal requests. In such a way, we provide a quantitative measure of the detected anomaly. 
    % An abnormal request is flagged if the anomaly score (as defined in Section \ref{sec:workflow}) exceeds a certain threshold.
\end{itemize}

We empirically validate that predictions made by \bp are more accurate than baseline solutions (in Section \ref{sec:model_compare}). We show that \bp can identify anomalous web requests (\eg, real-world exploits, widely-used web attacks) using the proposed quantitative measures (in Section \ref{sec:anomaly_eval}). We find these results encouraging and note that they highlight the benefit of analyzing web requests that co-occur within a context for anomaly detection. 

%In addition, in many cases especially in an Enterprise environment, as illustrated in Figure~\ref{fig:cross-apps}, users may need to make requests to different web applications to complete a specific task, or they access to a set of web applications regularly. Several web applications may compose a specific workflow. Therefore, the web requests generated by different web applications are not completely independent. This motivates us to design a context-based model from related web applications. As shown in Figure~\ref{fig:context-model}, we define the web application that has the event of interest as \textit{target app}, and its related web applications as \textit{exogenous apps}. 
% We refer the HTTP requests produced by the target web app as \textit{primary events}, and the ones produced by the exogenous web apps as \textit{contextual events}. 
%We combine requests from the target app and the exogenous apps as context and convert it to an embedding vector (Section~\ref{sec:model_context}).  To the best of our knowledge, this paper proposes the first approach to model the context for web requests from exogenous apps. 













==> 4_exo.tex <==
We observe the correlation between certain applications in the dataset. This indicates these applications are usually used together and perhaps for relevant work tasks in an enterprise environment. For example, in our experimental environment, users use Workqueue and DataAnalyzer1 together to complete one work task. 

%Because the rest applications do not ``interact'' with each other, we do not evaluate contextual events on them.
% \subsubsection{Context Modeling for Web requests of Correlated Web Applications}
% \label{sec:model_context}
% Analyzing a single application may bring a limited view of users' behavior. A user may make requests to multiple web applications. %Multiple web applications may compose a certain workflow. 
% We extend the proposed context-based model to have a comprehensive understanding of the multi-application environment. 
% To capture the contextual events from correlated web applications, we add an exogenous embedding layer to extract application information. Figure~\ref{fig:cross_em} shows an example of three embeddings: event embedding, sequence embedding, and exogenous embedding. For example, $e_1^t, e_2^t, e_3^t, e_4^t$ are contextual events from the target web application that we want to analyze. $e_1^1, e_2^1$ are contextual events from correlated web application $1$ and $e_1^2, e_2^2$ are contextual events from correlated web application $2$. As shown in the figure, we input an 8-event sequence: $\{e_1^t, e_2^t, e_1^1, e_2^1, e_3^t, e_1^2, e_2^2,e_4^t\}$ from both target and correlated applications. Same as the event embedding and sequence embedding described in Section~\ref{sec:workflow}, event embedding extracts the content of different events as $EE$, and sequence embedding extracts the location of events in the sequence as $SE$. In multi-application environment, we introduce exogenous embedding to add the indicators for different applications. Specifically, ``$XE=0$'' represents the event is from the target web application and ``$XE=i$'' represents the event is from the $i$th correlated web application. We extract three 128-dimensional vectors for event embedding $EE$, sequence embedding $SE$, and exogenous embedding $XE$, and sum them up as $em$. $em$ is the output of the embedding layer.
% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/cross_embedding.png}
% \caption{Embedding Layer with Contextual Events from Both Target Web Applications and Correlated Web Applications.}
% \label{fig:cross_em}
% \vspace{-0.5cm}
% \end{figure}
% In practice, correlated web applications may have many more events than the target web application. For instance, \bp ingests $W$ contextual events from the target application and correlated applications. $W$ denotes the window sizes of contextual events from each application. To avoid ``diluting'' events generated by the correlated web applications, \bp uses the most recent $W$ events from correlated applications and excludes the rest.

% \subsubsection{Evaluation on Contextual Events from Correlated Applications}
% In our dataset, Workqueue and DataAnalyzer1 are correlated, i.e., used together by users to accomplish work tasks. In our case, users use Workqueue to collect and analyze data and DataAnalyzer1 to report and visualize the analysis conducted by Workqueue. 
% To evaluate the impact of contextual events from correlated applications, we use Workqueue as the target application and DataAnalyzer1 as the correlated application, and vice versa. \bp ingests contextual events from both web applications and predicts the upcoming events of the target application. We report the results of \bp with the best settings (window size and with/without pre-training). We compare the performance of \bp with and without contextual events from the correlated application. 
% \begin{table}[tb]
% \centering
% \caption{Impact of Exogenous Embedding for Correlated Applications.}
% \label{tab:context}
% \small
% % \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{|c|c|c|}
% \hline
% \textbf{Application} & \textbf{Top-1}  & \textbf{Top-10}  \\ \hline
% \shortstack{Workqueue \\(no exogenous embedding)}    &75.21 & 99.27\\ \hline
% \shortstack{Workqueue \\(19.39\% events from DataAnalyzer1)}  & 78.53 & 99.22 \\ \hline
% \shortstack{DataAnalyzer1 \\(no exogenous embedding)}  & 70.10  & 95.44 \\ \hline
% \shortstack{DataAnalyzer1  \\(6.85\% events from Workqueue)} & 72.73  & 95.47 \\ \hline
% \end{tabular}
% \vspace{-0.5cm}
% \end{table}

% % Note that the exogenous ratio may not to be the same for Workque an due to their frequency and relative positions in the sequence. 

% As shown in Table~\ref{tab:context}, contextual events from correlated web applications help the prediction for target web applications in general. With the contextual events from correlated web applications, Top-1 accuracy increases from 75.21\% to 78.53\% for Workqueue, and 70.10\% to 72.73\% for DataAnalyzer1. 
% Exogenous embedding improves the prediction for both applications in terms of Top-1 accuracy, while does not change Top-10 accuracy much (less than 0.1\%). 
%We did not observe much improvement in Top-10.We observe that Top-10 accuracy for Workqueue decreases slightly (0.05\%) with exogenous embedding.

%In the table, we also note the average ratio of contextual events from correlated web application occurring in the input sequence. 
%The average ratio reflects how much events are used from the correlated web application. 
%Because DataAnalyzer1 contributes more contextual events to Workqueue than Workqueue contributes to DataAnalyzer1, \bp achieves more improvement on the predicting Workqueue events than DataAnalyzer1 events.

% We investigate the attention scores assigned to contextual events from target and exogenous apps using the first self-attention encoding layer. We set the window size to 128. Therefore we have at most 64 contextual events from target and exogenous apps each in an input sequence. We differentiate the scores assigned for target and exogenous app.

% Figure~\ref{fig:global_attention} illustrates the average attention scores assigned from the input sequence to the output sequence. First, we observe the majority of attention scores are assigned to the middle of the output sequence. In most cases, input sequence consists of 64 events from target app and only a few from exogenous app. Thus \bp mainly outputs around the middle of the output sequence, where the event of interest is located. 
% Second, higher attention scores are assigned to contextual events from target app other than exogenous app. We find that with more events from exogenous app (higher exogenous ratio), \bp attempts to assign higher attention scores. Workqueue as target app collects more contextual events than DataAnalyzer1, so that the events from exogenous app in Workqueue gains higher attention scores (comparing \ref{fig:global_1} with \ref{fig:global_2}). The higher attention scores in Workqueue suggests \bp learns more information from Workqueue's exogenous app than DataAnalyzer1. This explains why \bp achieves better performance improvement with more contextual events from exogenous apps.


% % the performance of \bp with contextual events is improved by applying pretraining techniques.
% \begin{figure}[!tb]
% \centering
% \begin{subfigure}{0.45\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figures/global_workqueueig_True1.png}
% \caption{Workqueue with DataAnalyzer1 (events from target app)}
% \end{subfigure}
% \begin{subfigure}{0.45\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figures/global_workqueueig_True2.png}
% \caption{Workqueue with DataAnalyzer1 (events from exogenous app)}
% \label{fig:global_1}
% \end{subfigure}
% \begin{subfigure}{0.45\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figures/global_igworkqueue_True1.png}
% \caption{DataAnalyzer1 with Workqueue (events from target app)}
% \end{subfigure}
% \begin{subfigure}{0.45\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figures/global_igworkqueue_True2.png}
% \caption{DataAnalyzer1 with Workqueue (events from exogenous app)}
% \label{fig:global_2}
% \end{subfigure}
% \caption{Attention Scores Assigned for Both Target and Exogenous App.}
% \label{fig:global_attention}
% \vspace{-0.5cm}
% \end{figure}




% We define an application as the primary application, which we predict the upcoming event, and the rest of applications as the contextual applications. We model the sequences in each contextual application by the same way as single-application \bp model. We input sequences from contextual application into each single-application \bp model. We consider the output of each contextual application as a new encoded event for the primary application. In practice, we encode the first output of each contextual application by a fully connected layer and output a 128-dimensional contextual embedding $c_k$. We append $K$ contextual embeddings to the embedding sequence $\{em_1, em_2, \ldots, em_n\}$ in primary application.

% \begin{figure}[!tb]
% \centering
% \includegraphics[width=0.95\linewidth]{figures/cross-bp.png}
% \caption{Modeling with Contextual Events from Both Target and Exogenous Apps.}
% \label{fig:cross_model}
% \vspace{-0.5cm}
% \end{figure}

% The settings of modeling the primary application and the contextual applications remain the same as Single-Application \bp model. 
% To remain Contextual Model consistent along different applications, we include the primary application in the contextual sequences. We force the primary application and other applications without any concurrent HTTP requests to output zero in their Contextual Models.

% \textbf{Exogenous Embedding}



==> results.tex <==







